Uniform Estimation and Inference for Nonparametric Partitioning-Based M-Estimators

This paper presents uniform estimation and inference theory for a large class of nonparametric partitioning-based M-estimators. The main theoretical results include: (i) uniform consistency for convex and non-convex objective functions; (ii) rate-optimal uniform Bahadur representations; (iii) rate-optimal uniform (and mean square) convergence rates; (iv) valid strong approximations and feasible uniform inference methods; and (v) extensions to functional transformations of underlying estimators. Uniformity is established over both the evaluation point of the nonparametric functional parameter and a Euclidean parameter indexing the class of loss functions. The results also account explicitly for the smoothness degree of the loss function (if any), and allow for a possibly non-identity (inverse) link function. We illustrate the theoretical and methodological results in four examples: quantile regression, distribution regression, $L_p$ regression, and logistic regression. Many other possibly non-smooth, nonlinear, generalized, robust M-estimation settings are covered by our results. We provide detailed comparisons with the existing literature and demonstrate substantive improvements: we achieve the best (in some cases optimal) known results under improved (in some cases minimal) requirements in terms of regularity conditions and side rate restrictions. The supplemental appendix reports complementary technical results that may be of independent interest, including a novel uniform strong approximation result based on Yurinskii's coupling.

==> main_paper_labels.tex <==
\prop_gset_from_keyval:Nn \g_main_paper_labels_prop
  {
    {sec:Introduction} = {1},
    {eq:Rhoproblem} = {1},
    {eq:Mestimator} = {2},
    {Assumption:gl-quasi-uniform-partition} = {A},
    {Assumption:gl-local-basis} = {B},
    {sec:Notation} = {1.4},
    {sec:MotivatingExamples} = {2},
    {example:GeneralizedConditionalQuantileRegression} = {1},
    {example:ConditionalDistributionRegression} = {2},
    {example:$L_p$regression} = {3},
    {example:Generalizedlinearmodels} = {4},
    {sec:Assumptions} = {3},
    {Assumption:dgp-holder} = {C},
    {Assumption:lossfunction} = {D},
    {shapeofderivative} = {\emph  {(iii)}},
    {Assumption:simplesetup} = {E},
    {Assumption:gl-approximation-error} = {F},
    {sec:consistency} = {4},
    {lem:consistency,convex} = {1},
    {eq:consistency,beta} = {3},
    {eq:consistency,sup} = {4},
    {eq:consistency,l2} = {5},
    {lem:consistency,nonconvex} = {2},
    {sec:WeakerConditionsforSpecialCases} = {4.3},
    {sec:ComparisonwithExistingResults--Consistency} = {4.4},
    {sec:Bahadurrepresentation} = {5},
    {theorem:bahadur-repres} = {1},
    {eq:Bahadurrep,disc} = {6},
    {eq:Bahadurrep,cont} = {7},
    {sec:ratesofconvergence} = {5.1},
    {coro:convergence} = {1},
    {eq:uniformconvergence} = {8},
    {coro:MeanSquareRateofConvergence} = {2},
    {eq:l2convergence} = {9},
    {sec:ComparisonwithExistingResults--Bahadur} = {5.2},
    {sec:uniforminference} = {6},
    {thm:strongapproximation} = {2},
    {eq:strongapprox,lipschitzcondition} = {\emph  {(iv)}},
    {sec:ComparisonwithExistingResults--SA} = {6.1},
    {sec:FeasibleUniformInference} = {7},
    {eq:feasiblecov} = {10},
    {thm:FeasiblePlug-inStrongApproximation} = {3},
    {eq:confidenceband} = {11},
    {sec:Examples} = {8},
    {sec:quantilereg} = {8.1},
    {lem:quantilereg} = {1},
    {sec:distributionreg} = {8.2},
    {lem:distributionreg} = {2},
    {sec:lpreg} = {8.3},
    {lem:lpreg} = {3},
    {sec:logitest} = {8.4},
    {lem:logitest} = {4},
    {sec:Extensions} = {9},
    {sec:conclusion} = {10},
  }


==> sa_labels.tex <==
\prop_gset_from_keyval:Nn \g_sa_labels_prop
  {
    {eq:holder-rho-problem} = {SA1.1},
    {eq:m-estimator} = {SA1.2},
    {eq:uniform-entropy-bound} = {SA1.3},
    {eq:def-subgaussian} = {SA1.4},
    {def:data} = {1},
    {eq:qbar-def} = {SA1.5},
    {eq:qzero-def} = {SA1.6},
    {eq:sigma-zero} = {SA1.7},
    {eq:sigma-bar} = {SA1.8},
    {eq:bigomega-def} = {SA1.9},
    {eq:bigomegabar-def} = {SA1.10},
    {sec:organization} = {SA1.2},
    {tab:CompareLit-Consistency} = {1},
    {tab:CompareLit-Bahadur} = {2},
    {tab:CompareLit-StrongApprox} = {3},
    {sec:setup} = {SA2},
    {ass:gl-quasi-uniform-partition} = {SA2.1},
    {ass:gl-local-basis} = {SA2.2},
    {ass:localization} = {(i)},
    {ass:well-conditioning} = {(ii)},
    {ass:basis-norm-bound} = {(iii)},
    {ass:dgp-holder} = {SA2.3},
    {ass:random-sample} = {(i)},
    {def:fx} = {2},
    {ass:cond-density} = {(iii)},
    {def:measureonY} = {3},
    {ass:mu-bounded} = {(iv)},
    {eq:ballqx-def} = {SA2.1},
    {ass:gl-holder} = {SA2.4},
    {ass:abs-cont} = {(i)},
    {def:riskder} = {4},
    {ass:psi-moments} = {(ii)},
    {def:riskderenvel} = {5},
    {ass:psi-holder-jumps} = {(iii)},
    {def:rangeeta} = {6},
    {eq:holder-assumption-with-cases-nonconvex} = {SA2.2},
    {eq:holder-assumption-without-cases-nonconvex} = {SA2.3},
    {ass:psi-eta} = {(iv)},
    {def:expriskder} = {7},
    {eq:PsiOneTwo} = {SA2.4},
    {ass:complexity} = {SA2.5},
    {ass:gl-approximation-error} = {SA2.6},
    {ass:gram-estimate} = {SA2.7},
    {def:qhat-rate} = {8},
    {ass:complexity-addition} = {SA2.8},
    {def:epsninassump} = {9},
    {sec:simpler-generalization-of-examples} = {SA2.1},
    {prop:simpler-generalization} = {SA2.9},
    {lem:simplified-class-g-one} = {SA2.10},
    {lem:simplified-class-g-two} = {SA2.11},
    {lem:simplified-class-g-three} = {SA2.12},
    {lem:simplified-class-g-four} = {SA2.13},
    {lem:simplified-class-g-five} = {SA2.14},
    {sec:simplified-example-verifying-addition-for-nonconvex-bahadur} = {SA2.1.2},
    {eq:nonconvex-complexity--verification-smooth-aux} = {SA2.5},
    {sec:preliminaries} = {SA3},
    {lem:subgaussian-max-bound} = {SA3.1},
    {lem:tech-stoch-orders-lemma} = {SA3.2},
    {lem:conv-to-zero-in-cond-p-equiv-to-conv-to-zero-in-p} = {SA3.3},
    {item:conv-to-zero-in-cond-p-equiv-to-conv-to-zero-in-p-1} = {(i)},
    {item:conv-to-zero-in-cond-p-equiv-to-conv-to-zero-in-p-2} = {(ii)},
    {lem:permanence-properties} = {SA3.4},
    {lem:maximal-ineq-gaussian-vectors} = {SA3.5},
    {lem:ueb-maximal-ineq} = {SA3.6},
    {lem:maximal-gaussian} = {SA3.7},
    {lem:closeness-in-prob-implies-closeness-of-cond-quantiles} = {SA3.8},
    {lem:anti-concentration-for-suprema-of-separable-gaussian-processes} = {SA3.9},
    {lem:mu-borel-measurable} = {SA3.10},
    {eq:mu-for-lp-reg-definition} = {SA3.1},
    {lem:holder-gram} = {SA3.11},
    {eq:q0q-eigenvalues-bound} = {SA3.2},
    {eq:q0q-inv-inf-norm-bound} = {SA3.3},
    {eq:qbarq-concentration} = {SA3.4},
    {eq:qbarq-eigenvalues-bound} = {SA3.5},
    {eq:qbarq-inv-inf-norm-bound} = {SA3.6},
    {eq:qbarq-inv-concentration} = {SA3.7},
    {eq:multiband-property} = {SA3.8},
    {eq:inv-multiband-exp-decay} = {SA3.9},
    {lem:holder-uniform-convergence-variance} = {SA3.12},
    {eq:uniform-convergence-variance-moment-case} = {SA3.10},
    {eq:uniform-convergence-variance-subgaussian-case} = {SA3.11},
    {eq:uniform-conv-variance-enough} = {SA3.12},
    {rem:rates-in-uniform-conv-var} = {SA3.13},
    {eq:XJQNHz} = {SA3.13},
    {lem:holder-projection-approximation-error} = {SA3.14},
    {eq:projection-approx-moment-case} = {SA3.14},
    {eq:a1q-conc} = {SA3.15},
    {eq:a2condexpbound} = {SA3.16},
    {eq:a2diffbound} = {SA3.17},
    {eq:projection-of-approx-variance} = {SA3.18},
    {eq:psi-difference-outside-segment} = {SA3.19},
    {eq:psi-difference-inside-segment} = {SA3.20},
    {eq:proj-of-approx-error-big-chain-restr-lebesgue-meas} = {SA3.21},
    {eq:proj-of-approx-error-big-chain-bounding-length} = {SA3.22},
    {eq:prof-of-approx-error-final-appl-of-gram-norm-lem} = {SA3.23},
    {rem:rates-in-proj-approx-error} = {SA3.15},
    {sec:consistency} = {SA4},
    {lem:holder-consistency} = {SA4.1},
    {eq:consistency-moment-case} = {SA4.1},
    {eq:consistency-subgaussian-case} = {SA4.2},
    {eq:beta-q-close-to-beta0} = {SA4.3},
    {eq:mu-est-close-to-mu0} = {SA4.4},
    {eq:l2-rate} = {SA4.5},
    {eq:holder-consistency-strategy} = {SA4.6},
    {eq:holder-consistency-delta-expectation-bound} = {SA4.7},
    {eq:holder-consistency-delta-concentration} = {SA4.8},
    {eq:holder-consistency-main-second-term-estimate} = {SA4.9},
    {lem:assumptions-of-nonconvex-consistency-are-reasonable} = {SA4.2},
    {eq:betazeroq-is-bounded-in-inf-norm} = {SA4.10},
    {deltaenvelopeboundauxtwo} = {1},
    {eq:rho-beta-minus-rho-betazeroq-bounded} = {SA4.11},
    {deltaenvelopeboundaux} = {2},
    {lem:consistency-nonconvex} = {SA4.3},
    {cond:cons-nonconvex-m-greater-half-d} = {(ii)},
    {cond:cons-nonconvex-rate-condition} = {(iii)},
    {eq:consistency-nonconvex-moment-case} = {SA4.12},
    {eq:consistency-nonconvex-subgaussian-case} = {SA4.13},
    {cond:lower-bound-of-psi-one} = {(v)},
    {cond:nonconvex-consistency-additional-complexity-assumption} = {(vi)},
    {deltacondauxone} = {4},
    {deltacondauxtwo} = {5},
    {deltacondone} = {6},
    {deltacondtwo} = {7},
    {lem:holder-consistency-unconnected} = {SA4.4},
    {eq:gram-matrices-restr-to-one-cell-eigen-bounds} = {SA4.14},
    {eq:holder-consistency-strategy-unconnected} = {SA4.15},
    {lem:nonconvex-cons-unconnected} = {SA4.5},
    {celldeltacondone} = {8},
    {celldeltacondauxtwo} = {9},
    {celldeltacondtwo} = {10},
    {lem:holder-consistency-strong-shape} = {SA4.6},
    {eq:strong-shape-gradient-diff} = {SA4.18},
    {eq:strong-shape-matrix-inf-norm-bound} = {SA4.19},
    {eq:strong-shape-grad-inf-norm-bound} = {SA4.20},
    {sec:bahadur-representation} = {SA5},
    {eq:bahterm-def} = {SA5.1},
    {th:bahadur-repres} = {SA5.1},
    {th:bahadur-repres-normal} = {(a)},
    {eq:bahadur-representation-conclusion-expr} = {SA5.2},
    {eq:bahadur-rates-for-statement} = {SA5.3},
    {th:bahadur-repres-cont} = {(b)},
    {eq:bahadur-representation-conclusion-expr-cont} = {SA5.4},
    {eq:bahadur-rates-for-statement-cont} = {SA5.5},
    {rem:qzero-vs-qbar} = {SA5.2},
    {sec:bahadur-representation-convex-proof} = {SA5.1},
    {eq:psuSJW} = {SA5.6},
    {eq:SdSOtN} = {SA5.7},
    {eq:bahbetabar-def} = {SA5.8},
    {eq:hgDEXQ} = {SA5.9},
    {eq:UMbHrv} = {SA5.10},
    {eq:bahadur-repres-last-step-subgradient-inequality} = {SA5.11},
    {eq:lqjlhq} = {SA5.12},
    {eq:term-delta-eta-one-bound-def} = {SA5.13},
    {eq:nnqhabbs0} = {SA5.14},
    {eq:nnqhabbs} = {SA5.15},
    {eq:qtilde-def} = {SA5.16},
    {eq:term-cond-exp-bound-def} = {SA5.17},
    {eq:term-delta-q-def} = {SA5.18},
    {eq:qqqhabb} = {SA5.19},
    {eq:term-delta-v-bound-def} = {SA5.20},
    {eq:bahadur-rtwo-def} = {SA5.21},
    {eq:bahadur-rone-def} = {SA5.22},
    {eq:two-lemmas-restrict-rone-strong} = {SA5.23},
    {def:betabarboundedevent} = {10},
    {eq:bahadur-bound-betabar} = {SA5.24},
    {space} = {1},
    {vbar} = {2},
    {neighborhood} = {3},
    {eq:eventi-def} = {SA5.25},
    {bahadur-var-bound} = {11},
    {difvvbar} = {4},
    {def:eventall} = {11},
    {eq:delta-eta1-bound-restr} = {SA5.26},
    {eq:JrjuDG} = {SA5.27},
    {eq:delta-q-bound-rate-restr} = {SA5.28},
    {lem:bahadur-concentration-of-g} = {SA5.3},
    {eq:bahadur-concentration-of-g} = {SA5.29},
    {conc} = {12},
    {eq:last-restr-first} = {SA5.30},
    {eq:last-restr-second} = {SA5.31},
    {eq:last-restr-third} = {SA5.32},
    {sec:bOVPpP} = {SA5.1.3},
    {locationl2} = {5},
    {locationl3} = {6},
    {eq:delta-q-i-after-dimension-considerations} = {SA5.33},
    {lem:bahadur-g-variance-bound} = {SA5.4},
    {lem:bahadur-g-complexity} = {SA5.5},
    {eq:log-d-entropy-chain} = {SA5.34},
    {lem:bahadur-delta-eta1-bound} = {SA5.6},
    {def:eventiii} = {12},
    {lem:bahadur-conditional-exp-bound} = {SA5.7},
    {lem:delta-q-bound-claim} = {SA5.8},
    {eq:delta-q-bound} = {SA5.35},
    {sec:bahadur-representation-nonconvex-proof} = {SA5.2},
    {lem:bahadur-nonconvex-g-variance-bound} = {SA5.10},
    {lem:bahadur-nonconvex-g-complexity} = {SA5.11},
    {lem:bahadur-nonconvex-concentration-of-g} = {SA5.12},
    {lem:nonconvex-delta-q-bound-claim} = {SA5.13},
    {def:qtildenonconv} = {13},
    {lem:nonconvex-bahadur-conditional-exp-bound} = {SA5.14},
    {lem:nonconvex-bahadur-delta-eta1-bound} = {SA5.15},
    {def:nonconvexeventiii} = {14},
    {cor:uniform-rate-of-convergence} = {SA5.16},
    {th:rates-of-conv-i} = {(a)},
    {eq:rates-lemma-uniform-rate} = {SA5.36},
    {eq:rates-lemma-additional-rate-restriction} = {SA5.37},
    {eq:rates-lemma-uniform-rate-modified} = {SA5.38},
    {cor:msq-rate-of-convergence} = {SA5.17},
    {eq:rates-lemma-additional-rate-restriction-for-l2} = {SA5.39},
    {eq:rates-lemma-l2-rate-modified} = {SA5.40},
    {eq:l2-beta-diff-norm-bound} = {SA5.41},
    {eq:l2-rates-diff-2norm-bound} = {SA5.42},
    {sec:strong-approximation} = {SA6},
    {sec:conditional-yurinskii-coupling} = {SA6.1},
    {th:cond-strassen} = {SA6.1},
    {th:conditional-yurinski} = {SA6.2},
    {eq:cond-yur-strassen-enough} = {SA6.1},
    {eq:cond-yur-rhs-with-f-dif} = {SA6.2},
    {lem:yurinski-coupling-K-dimensional} = {SA6.3},
    {def:ryur-in-yurinski-lemma} = {15},
    {eq:yurinski-lemma-rate-restriction} = {SA6.3},
    {eq:discretization-gn-final-bound} = {SA6.4},
    {covering} = {13},
    {eq:prelim-n-bound} = {SA6.5},
    {eq:discretization-zn-final-bound} = {SA6.6},
    {sec:SA-main-result} = {SA6.2},
    {eq:ellhatqx-def} = {SA6.7},
    {eq:elltwobarqx-def} = {SA6.8},
    {eq:ellqx-def} = {SA6.9},
    {eq:bartqx-def} = {SA6.10},
    {eq:hatTqx-def} = {SA6.11},
    {def:bigomegahat} = {16},
    {th:strong-approximation-binscatter-yurinski} = {SA6.4},
    {th:yurinski-normal} = {(a)},
    {eq:gRcohQ} = {SA6.12},
    {eq:yXRXnK} = {SA6.13},
    {eq:variance-closeness} = {SA6.14},
    {eq:l2-norm-holder-type-restriction} = {SA6.15},
    {def:yurinski-corollary-rate} = {17},
    {eq:MFPKjN} = {SA6.16},
    {def:gn} = {18},
    {def:zn} = {19},
    {eq:XcWykx} = {SA6.18},
    {eq:yurinski-corollary-statement} = {SA6.19},
    {eq:strong-approximation-t-process} = {SA6.20},
    {th:yurinski-subgauss} = {(b)},
    {def:yurinski-corollary-rate-subgauss} = {20},
    {eq:yurinski-corollary-statement-subgauss} = {SA6.21},
    {rem:strong-approx-correspondence} = {SA6.5},
    {lem:asympt-variance} = {SA6.6},
    {eq:bigomega-bounds} = {SA6.22},
    {eq:bigomega-and-bigomegabar-closeness} = {SA6.23},
    {eq:bigomegabar-bounds} = {SA6.24},
    {eq:bigomega-lower-bound} = {SA6.25},
    {lem:closeness-of-linear-terms} = {SA6.7},
    {eq:omega-inverse-root-diff-bound} = {SA6.26},
    {eq:omega-bar-inverse-root-diff-bound} = {SA6.27},
    {eq:ellqx-bound} = {SA6.28},
    {eq:elltwobardiff-bound} = {SA6.29},
    {eq:elltwobar-bound} = {SA6.30},
    {eq:ellhatdiff-bound} = {SA6.31},
    {eq:ellhat-bound} = {SA6.32},
    {eq:plug-in-two-terms} = {SA6.34},
    {lem:hats-off} = {SA6.8},
    {eq:rhatsoff-def} = {SA6.35},
    {eq:hats-off} = {SA6.36},
    {eq:TvfoLC} = {SA6.37},
    {sec:uniform-inference} = {SA7},
    {sec:plug-in} = {SA7.1},
    {eq:jvgoXA} = {SA7.1},
    {th:plug-in} = {SA7.1},
    {th:plug-in-cond-1} = {(i)},
    {th:plug-in-cond-3} = {(ii)},
    {eq:tJdMYD} = {SA7.2},
    {th:plug-in-cond-4} = {(iii)},
    {def:ScovEst} = {21},
    {eq:vJCqsc} = {SA7.3},
    {def:znhatst} = {22},
    {eq:feasible-vector-process} = {SA7.4},
    {def:znst} = {23},
    {eq:agGxAc} = {SA7.5},
    {eq:uBkMSP} = {SA7.6},
    {def:Rplugin} = {24},
    {rem:plug-in-correspondence} = {SA7.2},
    {sec:existence-of-feasible-process} = {SA7.1.2},
    {lqkjeh} = {14},
    {eq:large-event-lmax} = {SA7.7},
    {ahhQYwqt} = {15},
    {eq:uylQEQ} = {SA7.8},
    {eq:bMrBeR} = {SA7.9},
    {lem:solution-to-program} = {SA7.3},
    {def:SigmacovEstPlus} = {25},
    {lem:ANyFZe} = {SA7.4},
    {eq:VHEuxh} = {SA7.10},
    {lem:phBAhW} = {SA7.5},
    {def:zhatstpr} = {26},
    {eq:YHasPT} = {SA7.12},
    {lkjwh} = {16},
    {lem:bounding-the-sup-of-gaussian-process} = {SA7.6},
    {eq:prelim-n-bound-plug-in} = {SA7.13},
    {eq:Zq-Gaussian-maximal-bound} = {SA7.14},
    {eq:plug-in-first-term-bound} = {SA7.15},
    {eq:plug-in-second-term-bound} = {SA7.16},
    {th:confidence-bands} = {SA7.7},
    {def:k-star} = {27},
    {eq:cb-def} = {SA7.17},
    {eq:v-def} = {SA7.18},
    {eq:v-star-def} = {SA7.19},
    {eq:v-tilde-def} = {SA7.20},
    {eq:v-tilde-star-def} = {SA7.21},
    {def:k-star-tilde} = {28},
    {lem:v-rates} = {SA7.8},
    {lem:v-rates-v-v-tilde} = {(a)},
    {lem:v-rates-v-star-v-tilde} = {(b)},
    {lem:v-rates-v-bar-star-depends} = {(c)},
    {lem:conf-bands-quantiles-are-close} = {SA7.9},
    {lem:conf-bands-anti-concentration-of-v-tilde} = {SA7.10},
    {eq:quantile-diff-eq-one} = {SA7.22},
    {eq:quantile-diff-eq-two} = {SA7.23},
    {th:k-s-distance} = {SA7.11},
    {lem:OWTSYr} = {SA7.12},
    {eq:tildeZq-mean} = {SA7.25},
    {eq:tildeZq-closeness} = {SA7.26},
    {eq:tildeZqst-closeness} = {SA7.29},
    {eq:confidence-bands-t-z-bound} = {SA7.30},
    {eq:confidence-bands-z-z-hat-bound} = {SA7.31},
    {eq:confidence-bands-xi-eta-ineq} = {SA7.32},
    {eq:ellqx-z-is-close-to-ellqx-tildez} = {SA7.33},
    {eq:confidence-bands-xi-eta-deviation-from-const-bound} = {SA7.34},
    {eq:conf-bands-gaussian-concentration-chain} = {SA7.35},
    {eq:ellqx-zst-is-close-to-ellqx-tildezst} = {SA7.36},
    {sec:lem-OWTSYr-proof} = {SA7.3.1},
    {eq:mjWpbO} = {SA7.37},
    {lem:zptGdd} = {SA7.13},
    {def:tildeZpr} = {29},
    {eq:kynzOk} = {SA7.39},
    {eq:gSXmWZ} = {SA7.40},
    {sec:examples} = {SA8},
    {sec:example-quantile-regression} = {SA8.1},
    {prop:gl-holder-quantile-regression} = {SA8.1},
    {quant-compl-verification-a} = {17},
    {quant-compl-verification-v} = {18},
    {quant-compl-verification-envelope} = {19},
    {eq:quant-reg-compl-verification-uniform-entropy-bound} = {SA8.1},
    {quant-compl-verification-const-before-eps} = {20},
    {quantile-bounded-away-from-zero-const} = {21},
    {sec:example-distribution-regression} = {SA8.2},
    {prop:gl-holder-distribution-regression} = {SA8.3},
    {rem:feasibility-distr-reg} = {SA8.4},
    {eq:dist-reg-covariance-structure} = {SA8.2},
    {sec:distribution-regression-verifying-psi-holder-jumps} = {SA8.2},
    {sec:example-lp-regression} = {SA8.3},
    {prop:lp-regression} = {SA8.5},
    {eq:psi-int-goes-to-minus-inf} = {SA8.3},
    {eq:psi-int-goes-to-plus-inf} = {SA8.4},
    {eq:lp-reg-ggg-bound} = {SA8.5},
    {lp-reg-last-eps} = {22},
    {sec:example-logistic-regression} = {SA8.4},
    {prop:gl-holder-logistic-regression} = {SA8.6},
    {def:logRegPi} = {30},
    {eq:logistic-psi-one-eta-one-squared} = {SA8.6},
    {lem:logistic-entropy-one} = {SA8.7},
    {lem:logistic-entropy-two} = {SA8.8},
    {sec:examples-basis-functions} = {SA8.5},
    {sec:other-parameters-of-interest} = {SA9},
    {th:other-parameters} = {SA9.1},
    {other-params-one} = {(a)},
    {other-params-two} = {(b)},
    {other-params-three} = {(c)},
    {sec:simulation-evidence} = {SA10},
    {tab:m-def} = {4},
    {tab:dim1-point-small} = {5},
    {tab:dim1-uniform-small} = {6},
    {tab:dim2-point-small} = {7},
    {tab:dim2-uniform-small} = {8},
    {tab:dim1-point} = {9},
    {tab:dim1-uniform} = {10},
    {tab:dim2-point} = {11},
    {tab:dim2-uniform} = {12},
  }

